MCUBERT: Memory-Efficient BERT Inference on Commodity Microcontrollers

In this paper, we propose MCUBERT to enable language models like BERT on tiny microcontroller units (MCUs) through network and scheduling co-optimization. We observe the embedding table contributes to the major storage bottleneck for tiny BERT models. Hence, at the network level, we propose an MCU-aware two-stage neural architecture search algorithm based on clustered low-rank approximation for embedding compression. To reduce the inference memory requirements, we further propose a novel fine-grained MCU-friendly scheduling strategy. Through careful computation tiling and re-ordering as well as kernel design, we drastically increase the input sequence lengths supported on MCUs without any latency or accuracy penalty. MCUBERT reduces the parameter size of BERT-tiny and BERT-mini by 5.7$\times$ and 3.0$\times$ and the execution memory by 3.5$\times$ and 4.3$\times$, respectively. MCUBERT also achieves 1.5$\times$ latency reduction. For the first time, MCUBERT enables lightweight BERT models on commodity MCUs and processing more than 512 tokens with less than 256KB of memory.

==> docs/0-outline.tex <==
Introduction:
\begin{itemize}
    \item Background of VLN
    \item Background of VLN using LLM, compared with traditional works (training free, More extensive application scenarios)
    \item Problems of existing works: use ChatGPT-level model causing latency bottleneck
    \item Problems of directly using small VLM (challenges)
    \item We build a new method (observation and method)
    % \item Challenges of local LLaVa inference compared with chatgpt-level model inference
    \item Contributions (Accuracy, Latency, Memory)
\end{itemize}

Background and Motivation:
\begin{itemize}
    \item The two-stage inference structure of VLN (planner + controller). The importance of training-free LLM. 
    \item The structure of the navigation system. The bottleneck is LLM planner. ChatGPT-level model will bring concerns. 
    % Trand/natrual question prefilling: small model accuracy/latency
    \item The structure of the planner with navigation map, giving a global view.
    % \item The two-stage inference structure of VLN (planner + controller). The importance of training-free LLM. The bottleneck is VLM planner
    % \item The structure of the high-level planner, ChatGPT-level model will bring concerns. Trand/natrual question prefilling: small model accuracy/latency
    % \item The structure of the navigation map, giving a global view.
    % \item Visual-Language Navigation: importance of training-free
    % \item Zero-Shot Visual-Language Navigation: local inference and chatgpt-level work
    % \item Topomap description: importance of global view
\end{itemize}


% Challenge:
% \begin{itemize}
%     % \item An overview of our structure (LLaVa + topomap)
%     \item LLaVa is hard to deal with a complex navigation map.
%     \item A large number of nodes brings high prompt length. The sub-goal planning process becomes the main bottleneck, and LLaVa inference faces long prefill and decode latency
%     \item When using KV-cache, the GPU memory is limited.
% \end{itemize}

Challenge and Observation:
\begin{itemize}
    % \item An overview of our structure (LLaVa + topomap)
    \item LLaVa is hard to deal with a complex navigation map. While different nodes have different importance, so we can use pruning.
    \item We can use YOLO for environment description, so the sub-goal planning process becomes the main bottleneck. The sub-goal planning process becomes the main bottleneck. A large number of nodes brings high prompt length, and LLaVa inference faces long prefill and decode latency. We find that prefill is the latency bottleneck, so we use prompt cache to reduce prefill latency. When using prompt cache, the GPU memory is limited, so we use two-level storage system.
    \item The naive pipeline will bring high robot thinking time, which can not satisfy the real-time constraints.
%     LLaVa is hard to deal with a complex navigation map. While different nodes have different importance, so we can use
% pruning.
% • A large number of nodes brings high prompt length. The sub-goal planning process becomes the main bottleneck, and
% LLaVa inference faces long prefill and decode latency. We find prefill is the latency bottleneck, so we use prompt cache
% to reduce prefill latency. When using prompt cache, the GPU memory is limited, so we use two-level storage system.
% • The naive pipeline will bring high robot thinking time, which can not satisfy the real-time constraints
\end{itemize}

Overview:
\begin{itemize}
    \item We build a zero-shot local-inference navigation system using LLaVa for the first time.
    \item To improve LLaVa performance and accelerate the sub-goal planning process, we propose a node pruning method. This can make the planner pay more attention to the most important nodes.
    \item To accelerate the prefill stage in the sub-goal planning process, we propose a navigation-aware prompt cache system. To solve the high memory usage, we use two-level memory structure.
    \item System-level, we use pipeline, to reduce the robot thinking time.
\end{itemize}


% Observation:
% \begin{itemize}
%     \item Different nodes have different importance.
%     \item Sub-goal planning time is still long, and prefill stage is the bottleneck. Different nodes are independent to each other.
%     \item When the number of nodes becomes large, e.g. navigation in a factory, the storage of prompt cache for all nodes is unachievable as the GPU memory is limited. Loading cache from host memory will bring lower latency compared to re-computation.
%     \item The naive pipeline will bring high robot thinking time, which can not satisfy the real-time constraints.
% \end{itemize}

Method:
\begin{itemize}
    \item Instruction-aware Node pruning
    \item Navigation-aware Prompt cache
    \item Memory-computation-robot action system pipeline
\end{itemize}

Experiment Results:
\begin{itemize}
    \item SR and SPL comparison on Habitat-challenge
    \item Average latency compared with vllm 
    \item In different exploring step, the average latency of finding objects
    \item With different number of nodes, the prefill / decode latency of LLaVa inference on sub-goal planning

\end{itemize}

Ablation:
\begin{itemize}
    \item Average accuracy/latency with/without node pruning, prompt cache and pipeline
    \item Average accuracy/latency with different node pruning sparsity
    \item Average accuracy/latency with different node pruning strategies
    \item Average latency/memory on CPU offloading / re-computation
\end{itemize}


Problem:
\begin{itemize}
    % \item Why using LLaVA (real-time latency, privacy, energy)
    % \item Figures
    % \item instruction length
    % \item YOLO
    % \item Figure 19 stored
    % \item setup setting
    % \item planning latency?
    % \item Detection Latency
    % \item Node importance Observation
    % \item Ablation study
    % \item pipeline stage latency experiment
    \item do not storage some cache
    % \item navigation map will not change frequently (figure)
    % \item prefilling latency change to node description latency plus instruction latency (figure)

    \item performance
    % \item real-time or end-to-end
    \item in-door or not
    % \item Challenge2: planning latency
    % \item prompt cache or node cache
    % \item detection model or VLM
    \item VLM or LLM
\end{itemize}
